Autonomous Navigation in Unknown Environments with Sparse Bayesian Kernel-based Occupancy Mapping

This paper focuses on online occupancy mapping and real-time collision checking onboard an autonomous robot navigating in a large unknown environment. Commonly used voxel and octree map representations can be easily maintained in a small environment but have increasing memory requirements as the environment grows. We propose a fundamentally different approach for occupancy mapping, in which the boundary between occupied and free space is viewed as the decision boundary of a machine learning classifier. This work generalizes a kernel perceptron model which maintains a very sparse set of support vectors to represent the environment boundaries efficiently. We develop a probabilistic formulation based on Relevance Vector Machines, allowing robustness to measurement noise and probabilistic occupancy classification, supporting autonomous navigation. We provide an online training algorithm, updating the sparse Bayesian map incrementally from streaming range data, and an efficient collision-checking method for general curves, representing potential robot trajectories. The effectiveness of our mapping and collision checking algorithms is evaluated in tasks requiring autonomous robot navigation and active mapping in unknown environments.

==> tex/SparseKernelMap_backup.tex <==

\section{Summary on Sparse Kernel-based Occupancy Mapping and Autonomous Navigation}
\label{sec:kernel_map_summary}
In this section, we summarize our preliminary work \cite{duong2020autonomous} on sparse kernel-based occupancy mapping for completeness and for making connection with its Bayesian version developed in the subsequent sections. In particular, we proposed a novel mapping method that uses a kernel perceptron model to represent the occupied and free space of the environment. The model uses a set of support vectors to represent obstacle boundaries in configuration space. The complexity of this representation scales with the complexity of the obstacle boundaries rather than the environment size. We developed an online training algorithm to update the support vectors incrementally as new depth observations of the local surroundings are provided by the robot's sensors. To enable motion planning in the new occupancy representation, we developed an efficient collision checking algorithm for piecewise-linear and piecewise-polynomial trajectories in configuration space.

%\subsubsection{Sparse Kernel-based Occupancy Mapping}
Our training algorithm returns a set of $M^+$ positive support vectors and their weight $\Lambda^+ = \{(x_i, \alpha_i)\}$ and a set of $M^-$ negative support vectors and their weight $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$. A decision boundary is characterized by a score function 
\begin{equation}
\label{eq:fastron_score}
F(x) =\sum_{i = 1}^{M^+} \alpha_i^+ k(x_i^+, x) - \sum_{j = 1}^{M^-} \alpha_j^- k(x_j^-, x),
\end{equation}
where $k(\cdot, \cdot)$ is a kernel function and $\alpha_j^-, \alpha_i^+ > 0$. The occupancy of a query point $\bfx$ can be estimated from the support vectors by evaluating the score function $F(\bfx)$ in Eq.~\eqref{eq:fastron_score}. Specifically, $\hat{m}_t(\bfx) = -1$ if $F(\bfx) < 0$ and $\hat{m}_t(\bfx) = 1$ if $F(\bfx) \geq 0$.


 


%We propose a new version of the Fastron algorithm, utilizing only local streaming data, to achieve real-time sparse kernel-based occupancy mapping. For online learning, Fastron resamples a \textit{global} training dataset around the current support vectors and updates the support vectors. In our setting, only \textit{local} data in the robot's vicinity is available from the onboard sensors. We propose an incremental version of Fastron in Alg.~\ref{alg:fastron_model} such that: 1) training is performed with \textit{local} data $\mathcal{D}_t$ generated from a depth measurement $\bfz_t$ at a time $t$ and 2) the support vectors are stored in an $R^*$-tree data structure, enabling efficient score function~\eqref{eq:fastron_score} computations.


%\textbf{Data Generation}. Fig.~\ref{fig:laser_scan_ws} illustrates a lidar scan $\bfz_t$ obtained by the robot at time $t$. In configuration space, each laser ray end point corresponds to a ball-shaped obstacle, while the robot body becomes a point as shown in Fig.~\ref{fig:laser_scan_cs}. To generate local training data $\mathcal{D}_t$, the occupied and free C-space areas observed by the lidar are sampled (e.g., on a regular grid). As shown in Fig.~\ref{fig:orig_data}, this generates a set $\bar{\mathcal{D}}_t$ of points with label ``1'' (occupied) in the ball-shaped occupied areas and with label ``-1'' (free), outside. As unobserved areas are assumed free, neighboring points to the occupied samples in $\bar{\mathcal{D}}_t$ that are not already in $\bar{\mathcal{D}}_t$ or in the support vectors are added to an augmented set $\tilde{\mathcal{D}}_t$ with label ``-1''.    The augmented dataset $\tilde{\mathcal{D}}_t$ is illustrated in Fig.~\ref{fig:augmented_data} assuming the set of support vectors is empty. The local data $\mathcal{D}_t = \bar{\mathcal{D}}_t \cup \tilde{\mathcal{D}}_t$ (Fig.~\ref{fig:training_data}) is used in our Incremental Fastron Algorithm to update the support vectors (Fig.~\ref{fig:boundary_example}). Storing the sets of support vectors $\Lambda^+$, $\Lambda^-$ over time requires significantly less memory than storing the training data $\cup_t \mathcal{D}_t$. The occupancy of a query point $\bfx$ can be estimated from the support vectors by evaluating the score function $F(\bfx)$ in Eq.~\eqref{eq:fastron_score}. Specifically, $\hat{m}_t(\bfx) = -1$ if $F(\bfx) < 0$ and $\hat{m}_t(\bfx) = 1$ if $F(\bfx) \geq 0$. Fig.~\ref{fig:boundary_example} illustrates the boundaries generated by Alg.~\ref{alg:fastron_model}.

%\textbf{Score Approximation}. As the robot explores the environment, the number of support vectors required to represent the obstacle boundaries increases. Since the score function~\eqref{eq:fastron_score} depends on all support vectors, the time to train the kernel perceptron model online would increase as well. We propose an approximation to the score function $F(\bfx)$ under the assumption that the kernel function $k(\bfx_i, \bfx_j)$ is \emph{radial} (depends only on $\|\bfx_i-\bfx_j\|$) and \emph{monotone} (its value decreases as $\|\bfx_i-\bfx_j\|$ increases). To keep the presentation specific, we make the following assumption in the remainder of the paper.
%\begin{assumption*}
%$k(\bfx_i, \bfx_j) := \eta \exp\prl{-\gamma\|\bfx_i - \bfx_j\|^2}$
%\end{assumption*}
% A radial basis function kernel 
%  is used in Alg.~\ref{alg:fastron_model}.
%The kernel parameters $\eta, \gamma \in \mathbb{R}_{>0}$ can be optimized offline via automatic relevance determination~\cite{neal2012bayesian} using training data from known occupancy maps. 
%Our results also hold for an RBF kernel with elliptical level sets but we keep the form above to simplify the presentation. 
%The assumption implies that the value of $F(\bfx)$ is not affected significantly by support vectors far from $\bfx$. We introduce an $R^*$-tree data structure constructed from the sets of positive and negative support vectors $\Lambda^+$, $\Lambda^-$ to allow efficient $K$ nearest-neighbor lookup. The $K$ nearest support vectors, consisting of $K^+$ and $K^-$ positive and negative support vectors, are used to approximate the score $F(\bfx)$ (Lines 1-3 in Alg.~\ref{alg:fastron_model}).

%To make it more compatible with online mapping, an $R^*$-tree which allows efficient $K$ nearest-neighbor look up is used to store positive and negative support vectors separately. The $K^+$ and $K^-$ positive and negative support vectors are then used to calculate the score (Lines 2 and 3 in Algorithm \ref{alg:fastron_model}). This is motivated from the fact that the RBF kernel is negligible for farther support vectors.


A map representation is useful for navigation only if it allows checking a potential robot trajectory $\bfs(t)$ over time $t$ for collisions. We derived conditions for complete (without sampling) collision-checking of continuous-time trajectories $\bfs(t)$ in our sparse kernel-based occupancy map representation. Checking that a curve $\bfs(t)$ is collision-free is equivalent to verifying that $F(\bfs(t)) < 0$, $\forall t \geq 0$. It is not possible to express this condition for $t$ explicitly due to the nonlinearity of $F$. Instead, in Prop.~\ref{prop:score_bounds}, we show that an accurate upper bound $U(\bfs(t))$ of the score $F(\bfs(t))$ exists and can be used~to evaluate the condition $U(\bfs(t)) < 0$ explicitly in terms of $t$. The upper bound provides a conservative but fairly accurate ``inflated boundary'' and allows efficient collision checking for line segments and polynomial curves assuming a radial basis function kernel $k(\bfx, \bfx') = \eta \exp{(-\gamma \Vert \bfx - \bfx' \Vert^2)}$ is used.
\begin{proposition}
\label{prop:score_bounds}
For any $(\bfx_j^-, \alpha_j^-)\in \Lambda^-$, the score $F(\bfx)$ is bounded above by $U(\bfx)=k(\bfx, \bfx_*^+) \sum_{i = 1} ^ {M^+} \alpha^+_i \!-\! k(\bfx, \bfx_j^-)\alpha^-_j$ where $\bfx_{*}^{+}$ is the closest positive support vector to $\bfx$.
\end{proposition}

For line segments, suppose that the robot's path is described by a ray $\bfs(t) = \bfs_0 + t\bfv$, $t\geq 0$ such that $\bfs_0$ is obstacle-free, i.e., $U(\bfs_0) < 0$, and $\bfv$ is constant. To check if $\bfs(t)$ collides with the inflated boundary, we find the first time $t_u$ such that $U(\bfs(t_u)) \geq 0$. This means that $\bfs(t)$ is collision-free for $t \in [0,t_u)$. 
\begin{proposition}
%robot moves with a constant velocity $v$ starting from $s_0$ in the free region, i.e., $U(s_0) < 0$. The 
\label{prop:line_curve_defensive_checking} Consider a ray $\bfs(t) = \bfs_0 + t\bfv$, $t\geq 0$ with $U(\bfs_0) < 0$. Let $\bfx_i^+$ and $\bfx_j^-$ be arbitrary positive and negative support vectors. Then, any point $\bfs(t)$ is free as long as:

\begin{equation}
\label{eq:line_curve_t_condition}
t < t_u := \min_{i \in \{1, \ldots, M^+\}} \rho (\bfs_0, \bfx_i^+, \bfx_j^-)
\end{equation}
or
\begin{equation}
\label{eq:line_curve_t_condition_tigher_bound}
t <  t_u^* := \min_{i \in \{1, \ldots, M^+\}} \max_{j \in \{1, \ldots, M^-\}} \rho (\bfs_0, \bfx_i^+, \bfx_j^-).
\end{equation}
where $\beta = \frac{1}{\gamma}\left(\log (\alpha_j^-) - \log (\sum_{i = 1} ^ {M^+} \alpha_i^+)\right)$ and \\$\scaleMathLine[1.0]{\rho(\bfs_0, \bfx_i^+, \bfx_j^-) = 
\begin{cases} 
      +\infty, & \text{if}\ \bfv^T(\bfx_i^+ - \bfx_j^-) \leq 0  \\
      \frac{\beta - \Vert \bfs_0 - \bfx_j^-\Vert ^2 - \Vert \bfs_0 + \bfx_i^+ \Vert ^2}{2\bfv^T(\bfx_j^- - \bfx_i^+)}, & \text{if}\ \bfv^T(\bfx_i^+ - \bfx_j^-) > 0 
\end{cases}}$.
\end{proposition}
The computational complexities of calculating $t_u$ and $t^*_u$ are $O(M)$ and $O(M^2)$, respectively, where $M= M^+ + M^-$. Note that since often the robot's movement is limited to the neighborhood of its current position, $t_u$ can reasonably approximate $t^*_u$ if $\bfx_j^-$ is chosen as the negative support vector, closest to the current location $\bfs_0$. Calculation of $t_u$ in Eq.~\eqref{eq:line_curve_t_condition} is efficient in the sense that it has the same complexity as checking a point for collision ($O(M)$), yet it can evaluate the collision status for an entire line segment for $t \in [0, t_u)$ without sampling.  Collision checking becomes slower when the number of support vectors $M$ increases. We improve this further by using $K^+$ and $K^-$ nearest positive and negative support vectors instead of $M^+$ and $M^-$, respectively. Assuming $K^+$ and $K^-$ are constant, the computational complexities of calculating $t_u$ and $t^*_u$ reduce to $O(\log M)$ which is the complexity of an $R^*$-tree lookup.

In path planning, one often performs collision checking for a line segment $(\bfs_A, \bfs_B)$. All points on the segment can be expressed as $\bfs(t_A) = \bfs_A + t_A\bfv_A$, $\bfv_A = \bfs_B - \bfs_A$, $0 \leq t_A \leq 1$. Using the upper bound $t_{uA}$ on $t_A$ provided by Eq.~\eqref{eq:line_curve_t_condition} or Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}, we find the free regions $[0, t_{uA}]$ and $[0, t_{uB}]$ starting from $\bfs_A$ and $\bfs_B$, respectively. If the free regions overlap, the segment is free and vice versa.
\iffalse
\begin{algorithm}[h]
\caption{Line segment collision check}
\label{alg:collision_checking_line}
\footnotesize
	\begin{algorithmic}[1]	  
		\Require Line segment $(\bfs_A, \bfs_B)$; support vectors $\Lambda^+ = \{(\bfx_i^+, \alpha_i^+)\}$ and $\Lambda^- = \{(\bfx_j^-, \alpha_j^-)\}$
		%\Ensure True (Free) or False (Colliding)
		\State $\bfv_A = \bfs_B - \bfs_A$, $\bfv_B = \bfs_A - \bfs_B$
		\State Calculate $t_{uA}$ and $t_{uB}$ using Eq.~\eqref{eq:line_curve_t_condition} or Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}
    \If{$t_{uA} + t_{uB} > 1$} \Return True (Free)
		\Else \;\Return False (Colliding)
		\EndIf
	\end{algorithmic}
\end{algorithm}
\fi
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.5\linewidth]{fig/check_line_examples.pdf}\hfill%
%\includegraphics[width=0.49\linewidth]{fig/check_curve_examples.pdf}
%\caption{Collision checking for line segments (left), with bounds $t_{uA}$ and $t_{uB}$ obtained from Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}, and for second-order polynomial curves (right) using Euclidean balls.}
%\label{fig:collision_checking}
%\end{figure}
\iffalse
\begin{algorithm}[h!]
\caption{Polynomial curve collision check}
\label{alg:collision_checking_curve}
  \footnotesize
	\begin{algorithmic}
		\Require Polynomial curve $\bfs(t)$, $t \in [0,t_f]$; threshold $\varepsilon$; support vectors $\Lambda^+ = \{(\bfx_i^+, \alpha_i^+)\}$ and $\Lambda^- = \{(\bfx_j^-, \alpha_j^-)\}$, $k = 0$, $t_0 = 0$
		%Set of $M^+$ positive support vectors and their weight $\Lambda^+ = \{(x_i^+, \alpha_i^+)\}$; set of $M^-$ positive support vectors and their weight $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$, a polynomial curve $s(t), x(0) = s_0, x(1) = s_f, t \in [0,1]$, a threshold $\varepsilon$.
		%\Ensure True (Free) or False (Colliding)
		\While{True}
			\State Calculate $r_{k}$ using Eq. \eqref{eq:line_curve_radius} or Eq. \eqref{eq:line_curve_radius_star}.
			\If{$r_k < \varepsilon$} \Return False (Colliding)
			\EndIf
			\State Solve $\Vert \bfs(t) - \bfs(t_k) \Vert = r_k$ for $t_{k+1} \geq t_{k}$
			\If{$t_{k+1} \geq t_f$}
				\Return True (Free)
			\EndIf
		\EndWhile
	\end{algorithmic}
\end{algorithm}
\fi
%all points on the segment can also be expressed as $s(t_B) = s_B + t_Bv_B$, $v_B = s_A - s_B$, $0 \leq t_B \leq 1$. W
%, and find the free region on the line $AB$ starting from the endpoint $B$
%we consider the segment from endpoint $B$ and calculate an upper bound $t_{uB}$ on $t_B$ using Eq.~\eqref{eq:line_curve_t_condition} or Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}


%\begin{algorithm}
%\caption{Line Segment Collision Check}
%\label{alg:collision_checking_line}
%  \footnotesize
%	\begin{algorithmic}[1]
%		\Require Line segment $(s_A, s_B)$; positive and negative support vectors $\Lambda^+ = \{(x_i^+, \alpha_i^+)\}$, $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$
%%Set of $M^+$ positive support vectors and their weights $\Lambda^+ = \{(x_i^+, \alpha_i^+)\}$; set of $M^-$ positive support vectors and their weights $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$; line segment AB $(s_A, s_B)$.
%		\Ensure True (Free) or False (Colliding)
%		\State $v_A = s_B - s_A$, $v_B = s_A - s_B$
%		\State Calculate $t_{uA}$ and $t_{uB}$ using Eq.~\eqref{eq:line_curve_t_condition} or Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}
%				%\State Calculate $t_{uB}$ using Eq.  \eqref{eq:line_curve_t_condition} or  \eqref{eq:line_curve_t_condition_tigher_bound}
%		\If{$t_{uA} + t_{uB} > 1$} \Return True
%		\Else \;\Return False
%		\EndIf
%	\end{algorithmic}
%\end{algorithm}

%\begin{figure}[t]
%\centering
%\includegraphics[height=2.0in]{fig/check_line_examples.pdf} \hfill
%\includegraphics[height=2.0in]{fig/check_curve_examples.pdf}
%\caption{Collision checking for line segments with the bounds $t_{uA}$ and $t_{uB}$ calculated from Eq.~\eqref{eq:line_curve_t_condition_tigher_bound} (left) and second-order polynomial curves (right).}
%\label{fig:collision_checking}
%\end{figure}


%\begin{figure*}[t]
%\begin{minipage}{0.65\linewidth}
%\includegraphics[width=0.5\linewidth]{fig/check_line_examples.pdf}%
%\hfill%
%\includegraphics[width=0.49\linewidth]{fig/check_curve_examples.pdf}
%\caption{Collision checking for line segments with bounds $t_{uA}$ and $t_{uB}$ obtained from Eq.~\eqref{eq:line_curve_t_condition_tigher_bound} (left) and second-order polynomial curves (right).}
%\label{fig:collision_checking}
%\end{minipage}%
%\hfill%
%\begin{minipage}{0.34\linewidth}
%\vspace{-2ex}
%\begin{algorithm}[H]
%\caption{Line segment collision check}
%\label{alg:collision_checking_line}
%  \footnotesize
%	\begin{algorithmic}[1]
%		\Require Line segment $(s_A, s_B)$; support vectors $\Lambda^+ = \{(x_i^+, \alpha_i^+)\}$ and $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$
%		\Ensure True (Free) or False (Colliding)
%		\State $v_A = s_B - s_A$, $v_B = s_A - s_B$
%		\State Calculate $t_{uA}$ and $t_{uB}$ using Eq.~\eqref{eq:line_curve_t_condition} or Eq.~\eqref{eq:line_curve_t_condition_tigher_bound}
%    \If{$t_{uA} + t_{uB} > 1$} \Return True
%		\Else \;\Return False
%		\EndIf
%	\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{figure*}

We extend the collision checking algorithm for line segments by finding an Euclidean ball $\mathcal{B}(\bfs_0, r)$ around $\bfs_0$ whose interior is free of obstacles. 
%treating $\bfv$ as an arbitrary unit vector that may point in any direction and find a Euclidean ball $\mathcal{B}(\bfs_0, r)$ around $\bfs_0$ whose interior is free of obstacles. 
%of radius $r$
\begin{corollary}
\label{corollary:free_ball} Let $\bfs_0 \in \mathcal{C}$ be such that $U(\bfs_0) <0$ and let $\bfx_i^+$ and $\bfx_j^-$ be arbitrary positive and negative support vectors. Then, every point inside the Euclidean balls $\mathcal{B}(\bfs_0, r_u) \subseteq \mathcal{B}(\bfs_0, r_u^*)$ is free for:
\begin{align}
r_u &:= \min_{i \in \{1, \ldots, M^+\}} \bar{\rho}(\bfs_0, \bfx_i^+, \bfx_j^-) \label{eq:line_curve_radius}\\
r_u^* &:= \min_{i \in \{1, \ldots, M^+\}} \max_{j \in \{1, \ldots, M^-\}} \bar{\rho}(\bfs_0, \bfx_i^+, \bfx_j^-) \label{eq:line_curve_radius_star}
\end{align}
where $\bar{\rho}(\bfs_0, \bfx_i^+, \bfx_j^-) = \frac{\beta - \|\bfs_0 - \bfx_j^-\| ^2 + \|\bfs_0 - \bfx_i^+ \|^2}{2 \| \bfx_j^- - \bfx_i^+ \|}$ and $\beta = \frac{1}{\gamma} \prl{\log (\alpha_j^-) - \log (\sum_{i = 1} ^ {M^+} \alpha_i^+)}$.
\end{corollary}

Consider a polynomial $\bfs(t) = \bfs_0 + \bfa_1 t + \bfa_2 t^2 + \ldots + {\bfa}_d t^d$, $t \in [0, t_f]$  from $\bfs_0$ to $\bfs_f := \bfs(t_f)$. Corollary~\ref{corollary:free_ball} shows that all points inside $\mathcal{B}(\bfs_0, r)$ are free for $r = r_u$ or $r^*_u$. If we can find the smallest positive $t_1$ such that $\|\bfs(t_1) - \bfs_0 \| = r$, then all points on the curve $\bfs(t)$ for $t \in [0, t_1)$ are free. We perform collision checking by iteratively covering the curve by Euclidean balls. If the radius of any ball is smaller than a threshold $\varepsilon$, the curve is considered colliding. Otherwise, the curve is considered free. 

%The collision checking process for $d$-order polynomial curves is shown in Alg.~\ref{alg:collision_checking_curve}. 

%Finally, we present a complete online mapping and navigation approach that solves Problem~\ref{problem_formulation_unknown_env}. 
Given the kernel-based map $\hat{m}_{t_k}$, a motion planning algorithm such as $A^*$~\cite{Russell_AI_Modern_Approach} may be used with our collision-checking algorithms to generate a path that solves the autonomous navigation problem. The robot follows the path for some time and updates the map estimate $\hat{m}_{t_{k+1}}$ with new observations. Using the updated map, the robot re-plans the path and follows the new path instead.
% This process is repeated until the goal is reached or a time limit is exceeded (Alg.~\ref{alg:auto_nav_fastron_ogm}).
% summarizes the autonomous navigation approach.
%(see Alg.~\ref{alg:get_successors})
\iffalse
\begin{algorithm}[t]
\caption{getSuccessors subroutine in $A^*$}
\label{alg:get_successors}
  \footnotesize
	\begin{algorithmic}[h!]
		\Require Current position $\bfs$; neighbor threshold $\delta$; support vectors $\Lambda^+ = \{(\bfx_i^+, \alpha_i^+)\}$ and $\Lambda^- = \{(\bfx_j^-, \alpha_j^-)\}$ 
		%Set of $M^+$ positive support vectors and their weight $\Lambda^+ = \{(x_i, \alpha_i)\}$; set of $M^-$ positive support vectors and their weight $\Lambda^- = \{(x_j^-, \alpha_j^-)\}$, current cell $x$, $S = \emptyset$, neighbor threshold $\delta$.
		%\Ensure Set of successors $S$.
		\State $S \gets \emptyset$; Find potential successors $\mathcal{N}(\bfs) = \{\bfs'\in \bar{\mathcal{C}}: \| \bfs' -\bfs \|_\infty \leq \delta\}$
		\For{$\bfs'$ in $\mathcal{N}(\bfs)$}
			\If{Check Line Segment$(\bfs, \bfs',\Lambda^+ ,\Lambda^-)$} \Comment{Alg.~\ref{alg:collision_checking_line}} % Check if segment $(\bfs,\bfs')$ is free (
				\State $S \leftarrow S \cup \{\bfx'\}$
			\EndIf
		\EndFor
		\State \Return Set of successors $S$
	\end{algorithmic}
\end{algorithm}
\fi

%We consider robots with two different motion models. In simulation, we use a first-order fully actuated robot, $\dot{\bfs} = \bfv$, with piecewise-constant velocity $\bfv(t) \equiv \bfv_k \in \calV$ for $t \in [t_k,\;t_{k+1})$, leading to piecewise-linear trajectories. In real experiments, we consider a ground wheeled Ackermann-drive robot whose dynamics can be transformed into a 2nd-order fully actuated system $\ddot{\bfs} = \bfa$ via feedback linearization~\cite{de2000stabilization, franch2009control}. Using piecewise-constant acceleration $\bfa(t) \equiv \bfa_k \in \calA$ for $t \in [t_k,\;t_{k+1})$ leads to piecewise-2nd-order-polynomial trajectories. 

%The experiments shows the effectiveness of our mapping and collision checking algorithms. We showed that the memory requirements of our mapping method is comparable to those of OctoMap as both ours and OctoMap depends on the complexity of the obstacle boundaries. As our collision checking method can check linear and polynomial trajectories without the need to sample, we showed that our collision checking time stay flat while sampling based checking time increases as the number of samples and/or the trajectory length increases. We demonstrated our approach for online mapping and autonomous navigation on a real ground robot in real time.


Our kernel-perceptron-based mapping method and collision checking algorithms are evaluated in both simulated and real experiments. In our experiments, we observed that kernel-based mapping is susceptible to noise and localization errors since the support vectors are quickly updated with newly observed data.  \TD{(They might ask us to provide quantitative comparison showing that our Bayesian version is better with noise???)} This is caused by the kernel perceptron model not maintaining occupancy probabilities. Therefore, in this work, we focus on sparse probabilistic models for occupancy maps and development of efficient collision checking algorithms for the proposed probabilistic map representation.









